TractoGPT: A GPT architecture for White Matter Segmentation

White matter bundle segmentation is crucial for studying brain structural connectivity, neurosurgical planning, and neurological disorders. White Matter Segmentation remains challenging due to structural similarity in streamlines, subject variability, symmetry in 2 hemispheres, etc. To address these challenges, we propose TractoGPT, a GPT-based architecture trained on streamline, cluster, and fusion data representations separately. TractoGPT is a fully-automatic method that generalizes across datasets and retains shape information of the white matter bundles. Experiments also show that TractoGPT outperforms state-of-the-art methods on average DICE, Overlap and Overreach scores. We use TractoInferno and 105HCP datasets and validate generalization across dataset.

==> sections/intro.tex <==
Fiber tract segmentation is a pivotal process in Neuroimaging, enabling detailed analysis of White Matter connectivity through Diffusion Magnetic Resonance Imaging (dMRI).
Tractography traces the anisotropic diffusion of water molecules along neural pathways, yielding three-dimensional streamlines that represent white matter fiber bundles. 
These streamlines are grouped into specific anatomical tracts, providing crucial insights into brain connectivity and function, essential for understanding development, aging, and neurological conditions \cite{basser1994mr}.
%Diffusion Magnetic Resonance Imaging (dMRI) is an essential tool in neuroimaging, enabling non-invasive mapping of the human brain by tracking the anisotropic movement of water molecules along neuronal pathways. 
%This process generates a three-dimensional sequence of coordinates which are white matter streamlines. Streamlines are grouped into anatomical connections known as white matter tracts, essential for understanding brain connectivity and function \cite{basser1994mr}. 
With recent advancements, fiber tract segmentation methods can be broadly categorized into classical and deep learning techniques. Classical methods, such as \textit{QuickBundles} and \textit{QuickBundlesX}, use Mean Direct-Flip Distance (MDF) to cluster streamlines into bundles or tracts \cite{garyfallidis2012quickbundles}. 
Other Techniques, like \textit{WMA} \cite{o2012unbiased}, incorporate anatomical priors, while  RecoBundles \cite{garyfallidis2018recognition} recognizes model bundles, and BundleSeg \cite{st2023bundleseg} enhances this recognition within target tracts via Fast Streamline Search. 
Deep learning Tract Segmentation approaches, for instance, TractSeg \cite{wasserthal2018tractseg} employs Convolutional Neural Networks (CNNs) across multiple MRI slices, and DeepWMA \cite{zhang2020deep} utilizes novel fiber descriptors.
Additionally, clustering techniques like CINTA \cite{legarreta2022clustering} leverage streamline clustering, and FINTA \cite{legarreta2021filtering} does filtering in embedding space, and FIESTA \cite{dumais2023fiesta} further improves the performance by employing autoencoders to segment and filter streamlines in latent space through FINTA multibundles, then generating additional streamlines with GESTA-GMM \cite{legarreta2023generative} to fill bundles and meet semi-automatically calibrated bundle-specific thresholds.
Recent tract segmentation studies have also explored point cloud networks \cite{xue2023tractcloud, xue2023superficial, goel2024tractoembed}. But many methods stated above either require registration, ATLAS, filtering or calibration for thresholds.
In this paper, 
\begin{itemize} 
\item We introduce \textbf{TractoGPT}, a novel, fully-automatic, \textbf{registration-free} white matter segmentation network inspired by the GPT architecture using auto-regressive pretraining.
\item In addition to TractoGPT framework, we introduce a\\ \textbf{Fusion} Data Representation which enhances representation for tractography streamline data for downstream segmentation task. 
\item TractoGPT also \textbf{generalizes across datasets} and retains shape information of major White Matter Bundles. 
\end{itemize}




==> sections/model.tex <==
We employ an autoregressive pre-training strategy to streamline and cluster data. We consider streamline or cluster as point clouds randomly sampled 1024 points. After the point patches are extracted from \textit{FPS kNN}, we consider each patch as a token, and generate token embedding using a mini-pointnet \cite{}, to make a sequence of tokens. 
We preserve the sequential information of the point cloud and do not shuffle the sequence of point patches. 
Training of GPT model is done by an encoder with extracts magnitude and direction information from the token embeddings and 

\textbf{Point Patch Partitioning}: The input point cloud X with M points is processed using Farthest Point Sampling (FPS) and K-Nearest Neighbors (KNN) to get center points and point patches. First, n center points are sampled from X using FPS. Then, KNN is applied to select the k-nearest neighbors for each center point, forming n point patches. The patches are created to overlap, ensuring the retention of continuous information across the point cloud. 

\textbf{Sorting}: Point patches are organized into a sequence based on their center points. The coordinates of the center points are first encoded into a one-dimensional space using Morton code, and then sorted to determine the order of center points. The point patches are subsequently arranged according to this order.

\textbf{Embedding}: A MiniPointNet network is used to extract features from each point patch. For better training convergence, the coordinates of each point are normalized relative to its center point before they are fed to MiniPointNet.



\textbf{Transformer Decoder}: A dual masking strategy is employed to enhance the comprehensive understanding of point clouds. An extractor-generator transformer architecture is used, where the generator focuses on the generation task and is discarded after pre-training. This process improves the semantic quality of the latent representations learned by the extractor.

\textbf{Dual Masking Strategy}: To promote the learning of more useful representations, a dual masking strategy is applied. In addition to masking input tokens, a proportion of the preceding tokens attending to each token is also masked during pre-training. 

\textbf{Extractor-Generator:} The extractor consists of transformer decoder blocks utilizing a dual masking strategy to generate latent representations, where each point token attends only to the unmasked preceding tokens. Since point patches are represented in normalized coordinates and global structures are critical for point cloud understanding, sinusoidal positional encodings (PE) are applied to map the coordinates of the sorted center points CsC\_sCs to absolute positional encoding (APE). These positional encodings are added to each transformer block to provide location information and incorporate global structural context. 

The generator architecture mirrors that of the extractor but consists of fewer transformer blocks. It receives the extracted tokens as input and generates point tokens for the prediction head. However, the order of patches can be influenced by the center point sampling process, leading to ambiguity in predicting subsequent patches. This ambiguity hampers the model's ability to learn meaningful representations of point clouds. To mitigate this issue, the generator incorporates directions relative to the subsequent point patches as prompts, without disclosing the locations of masked patches or the overall shapes of the point clouds. 

\textbf{Prediction Head:} The prediction head is designed to predict subsequent point patches in the coordinate space. It comprises a two-layer multi-layer perceptron (MLP) featuring two fully connected (FC) layers and utilizes rectified linear unit (ReLU) activation functions. 

Generation Target: The goal for each point patch is to predict the coordinates of the points in the subsequent patches. The generation loss is calculated using both the L1-form and L2-form of the Chamfer Distance (CD).




==> sections/training.tex <==
\begin{itemize}
    \item Train: per subject: per class; 250 streamlines (totalling $n_{sub}$ *250)
    \item Test: per subject: all of the streamlines for all bundles 
\end{itemize}

In the model training and testing strategy for TractoGPT, we implement a comprehensive approach that includes pretraining, fine-tuning, and testing, as detailed in the PointGPT paper. \\
\textbf{Pretraining} involves using a 50:50 Chamfer Loss (L1 and L2) without labels, optimized with AdamW (weight decay of 0.05) and a cosine learning rate scheduler starting at 0.0001 over 300 epochs with a batch size of 250 on a single streamline setup using a 16GB V100 GPU, which takes approximately 24 hours. Various hybrid configurations are tested, including different batch sizes and dimensions (e.g., 256 and 1024) across multiple clusters like QBX and Fusion. \\
In \textbf{fine-tuning}, we employ a combination of Cross Entropy and Chamfer Distance Loss (CDL), adjusting batch sizes according to the model type (Hybrid, TF, HCP). 
The training utilizes designated train, validation, and test splits from the TractoInferno dataset to ensure robust evaluation.
The overall strategy is designed to optimize the model's performance in streamline reconstruction tasks while leveraging advanced loss functions such as Chamfer Distance for effective point cloud completion

==> tables/hcp_results.tex <==
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}\hline
\textbf{Data Rep} & \textbf{Model} & \textbf{DICE score} & \textbf{OvL} & \textbf{OvR} & \textbf{Bundle similarity (599469)} & \textbf{Accuracy} \\\hline
\multirow{2}{*}{\textbf{Streamline}} & \textbf{mini} & 0.1753 ± 0.1526 & 0.2469 ± 0.2020 & 19.1248 ± 62.5817 & 0.1371 ± 0.1732 & 12.48\% \\\cline{2-7}
& \textbf{small} & 0.1991 ± 0.1616 & 0.3227 ± 0.2518 & 24.7712 ± 60.7986 & 0.1985 ± 0.1774 & 17.22\% \\\hline
\multirow{2}{*}{\textbf{Cluster}} & \textbf{mini} & 0.8333 ± 0.1964 & 0.7706 ± 0.2202 & 0.0255 ± 0.0378 & 0.8572 ± 0.1511 & 87.60\% \\\cline{2-7}
& \textbf{small} & 0.8296 ± 0.2048 & 0.7675 ± 0.2318 & 0.0237 ± 0.0315 & 0.8618 ± 0.1432 & 87.66\% \\\hline
\multirow{2}{*}{\textbf{Fusion}} & \textbf{mini} & 0.8333 ± 0.1763 & 0.7611 ± 0.2003 & 0.0213 ± 0.0442 & 0.8626 ± 0.1290 & 87.57\% \\\cline{2-7}
& \textbf{small} & 0.8476 ± 0.1567 & 0.7731 ± 0.1835 & 0.0147 ± 0.0157 & 0.8715 ± 0.1132 & 88.41\% \\\hline
\end{tabular}
\end{table}


==> tables/hybrid_results.tex <==
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}\hline
\textbf{Data Rep} & \textbf{Model} & \textbf{DICE score} & \textbf{OvL} & \textbf{OvR} & \textbf{Bundle similarity(599469)} & \textbf{Accuracy} \\\hline
\multirow{2}{*}{\textbf{Streamline}} & \textbf{mini} & 0.1753 +- 0.1526 & 0.2469 +- 0.2020 & 19.1248 +- 62.5817 & 0.1371 +- 0.1732 & 12.48\% \\ \cline{2-7}
& \textbf{small} & 0.1991 +- 0.1616 & 0.3227 +- 0.2518 & 24.7712 +- 60.7986 & 0.1985 +- 0.1774 & 17.22\% \\ \hline
\multirow{2}{*}{\textbf{Cluster}} & \textbf{mini} & 0.8333 +- 0.1964 & 0.7706 +- 0.2202 & 0.0255 +- 0.0378 & 0.8572 +- 0.1511 & 87.60\% \\ \cline{2-7}
& \textbf{small} & 0.8296 +- 0.2048 & 0.7675 +- 0.2318 & 0.0237 +- 0.0315 & 0.8618 +- 0.1432 & 87.66\% \\ \hline
\multirow{2}{*}{\textbf{Fusion}} & \textbf{mini} & 0.8333 +- 0.1763 & 0.7611 +- 0.2003 & 0.0213 +- 0.0442 & 0.8626 +- 0.1290 & 87.57\% \\ \cline{2-7}
& \textbf{small} & 0.8476 +- 0.1567 & 0.7731 +- 0.1835 & 0.0147 +- 0.0157 & 0.8715 +- 0.1132 & 88.41\% \\ \hline
\end{tabular}
\end{table}


==> tables/tf_results.tex <==
\begin{table}[!htp]
\centering
\caption{Generated by Spread-LaTeX}
\label{tab: }
\begin{tabular}{|l|r|r|r|r|} % Adjusted column specification
\hline
\textbf{Data Rep} & \textbf{Model} & \textbf{DICE score} & \textbf{OvL} & \textbf{Accuracy} \\ % Removed BS(sub-1006)
\hline
\multirow{2}{*}{\textbf{Streamline}} & \textbf{mini} & 0.88 ± 0.07 & 0.82 ± 0.11 & 84.28\% \\
\cline{2-5}
& \textbf{small} & 0.88 ± 0.07 & 0.82 ± 0.11 & 84.39\% \\
\hline
\multirow{2}{*}{\textbf{Cluster}} & \textbf{mini} & 0.96 ± 0.04 & 0.96 ± 0.03 & 88.31\% \\
\cline{2-5}
& \textbf{small} & 0.96 ± 0.04 & 0.96 ± 0.04 & 87.89\% \\
\hline
\multirow{2}{*}{\textbf{Fusion}} & \textbf{mini} & 0.95 ± 0.04 & 0.95 ± 0.04 & 87.87\% \\
\cline{2-5}
& \textbf{small} & 0.95 ± 0.04 & 0.94 ± 0.05 & 88.00\% \\
\hline
\end{tabular}
\end{table}

